A Predictive Approach to Bayesian Nonparametric Survival Analysis

Bayesian nonparametric methods are a popular choice for analysing survival data due to their ability to flexibly model the distribution of survival times. These methods typically employ a nonparametric prior on the survival function that is conjugate with respect to right-censored data. Eliciting these priors, particularly in the presence of covariates, can be challenging and inference typically relies on computationally intensive Markov chain Monte Carlo schemes. In this paper, we build on recent work that recasts Bayesian inference as assigning a predictive distribution on the unseen values of a population conditional on the observed samples, thus avoiding the need to specify a complex prior. We describe a copula-based predictive update which admits a scalable sequential importance sampling algorithm to perform inference that properly accounts for right-censoring. We provide theoretical justification through an extension of Doob's consistency theorem and illustrate the method on a number of simulated and real data sets, including an example with covariates. Our approach enables analysts to perform Bayesian nonparametric inference through only the specification of a predictive distribution.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> preamble.tex <==

\definecolor{ef}{rgb}{.0, .5, .75}
\definecolor{bl}{rgb}{.5, .25, .75}
\definecolor{ch}{rgb}{.5, 0, .5}

\newcommand{\ch}[1]{{{\color{purple}Chris: [#1]}}}
\newcommand{\ef}{\textcolor{ef}{Edwin\ }}
\newcommand{\bl}{\textcolor{bl}{Brieuc\ }}


\newcommand{\eft}[1]{\textcolor{ef}{[\ef: #1]}}
\newcommand{\blt}[1]{\textcolor{bl}{[\bl: #1]}}
\newcommand{\cht}[1]{\textcolor{ch}{[\ch: #1]}}

